Generic Torelli and local Schottky theorems for Jacobian elliptic surfaces

We prove a generic Torelli theorem for Jacobian elliptic surfaces, provided that the geometric genus is large compared to the irregularity. The result is effective to the extent that defining equations for the base curve are recovered from the period data.

==> Dynkin.tex <==
%%   This package draws the Dynkin and extended Dynkin graphs in the
%%   simply laced case (A, D and E) with the exception of the A~ class.
%%   The appropriate control sequences are \dynkinA, \dynkinD, \dynkinE,
%%   \dynkinDtilde, and \dynkinEtilde. They all take a numerical argument
%%   which is separated with a space from following text. The vertices of the
%%   graphs are drawn with a macro \dynkinball which can be redefined by the
%%   user. See the option dotchoice below for details.
%%   
%%       There are several options, which all are set by the \setdynkin macro:
%%   
%%   \setdynkin size=.5cm<space> 
%%   
%%     sets the length of the horisontal and vertical edges. Any dimension
%%     specification acceptable by TeX is allowed where .5cm was put in the
%%     example. 1 cm is the default.
%%   
%%   \setdynkin slope="25<space>
%%   
%%     sets the characters of the line10 font to use for sloped edges in D and
%%     D~.  The argument, here "25, is the character for upwards slope and the
%%     corresponding for downwards slope is computed by adding 64 to it (which
%%     seems to be line10's encoding). The default value is 0.
%%   
%%   \setdynkin lines=1<space>
%%   
%%     sets the number of lines to use for the sloped edges. Currently only 1 or
%%     2 are possible and 2 is the default.
%%   
%%   \setdynkin dotchoice=y<space>
%%   
%%     sets whether or not it should be possible to use different types of
%%     vertices at different positions. The choices are y for yes and n for no
%%     (the default).  If y is set then the \dynkinball should take one argument
%%     and the graph drawing macros \dynkinA etc will take more than the numeric
%%     arguments. More precisely:
%%   
%%       If dotchoice is set and tags is not (see below) then the supplementary
%%       argument is a space-separated list of items, one for each vertex of the
%%       graph. These items then passed to the macro \dynkinball which then
%%       decides what type of edge to draw. The order in which the edges are
%%       drawn is as follows:
%%            For A the vertices are drawn form left to right.
%%            For D the vertices on the horisontal line are drawn 
%%          from left to right, then the upper vertex of the right 
%%          fork and finally the lower vertex of that fork.
%%            For D~ the the upper vertex of the left fork is drawn 
%%          first, then the lower vertex of that fork is drawn, then 
%%          the vertices on the horisontal line from left to right, 
%%          then the upper vertex of the right fork and finally the
%%          lower vertex of that fork.
%%            For E and  E~ the vertices are drawn from left to right
%%          and from the bottom to the top. Thus for E, for instance,
%%          first three vertices on the horisontal line are drawn,
%%          then the uppermost vertex and then finally the rest of 
%%          horisontal vertices.
%%       If dotchoice and tags is set then the supplementary arguement
%%       is a space-separated list of pairs of items, one such pair for each 
%%       vertex, the items are separated by a comma and the first item is
%%       passed to \dynkinball and the second will be placed near the edge
%%       on the drawn graph.
%%   
%%       Example:
%%         \setdynkin dotchoice=y \setdynkin tags=y
%%         \dynkinE 8 c,1 b,2 c,3 b,4 c,5 b,6 c,7 b,8
%%       This will mark the vertices with consecutive numbers and
%%       consecutively pass c, b, c, b, c, b, c, and b to \dynkinball.
%%   
%%     Note that the package will call \dynkinball once before actually
%%     drawing anything with the first item as argument and use that
%%     result to determine the extent of all the vertices. Hence it is
%%     not a good idea to make the vertices of different size.
%%     Three \dynkinball macros are provided. See \setdynkin ball below.
%%   
%%   \setdynkin tags=y<space>
%%   
%%     sets whether or not tags should be put close to each vertex. The
%%     arguments are y for yes and n for no (the default). The tags
%%     are specified as a space-separated list. When dotchoice is also
%%     the format for that list has already been described, when not the
%%     items are simply used.
%%   
%%   \setdynkin ball=bullet<space>
%%   
%%    sets \dynkinball to one of three predefined macros. The possibilities
%%    are
%%      ball=bullet  (the default)
%%       will set \dynkinball to a parameterless macro which produces a
%%       bullet ($\bullet$).
%%      ball=bulletandcirc
%%       will set  \dynkinball to a macro taking one argument which
%%       produces a bullet if the argument is b and a circle ($\circ$)
%%       if the argument is a c.
%%      ball=bigcirc
%%       will set \dynkinball to a parameterless macro which produces a
%%       big circle ($\bigcirc$).
%%    (Note that in all cases the box in which these characters are put
%%    is slightly bigger than the characters themselves which forces
%%    some adjustment as can be seen from the macros.

\catcode`\@=11
\let\e@\expandafter
\def\d@nkinsize{1cm}
\newcount\d@nkincount
\d@nkincount"00
\newif\if@ne

\def\LINE{\hbox to \hsize}
\def\setdynkin#1=#2 {\csname d@nkin@#1\endcsname{#2}}
\def\d@nkin@size#1{\def\d@nkinsize{#1}}
\def\d@nkin@slope#1{\d@nkincount#1}
\def\d@nkin@lines#1{\ifnum#1=1\@netrue\else\@nefalse\fi}
\newif\ifd@dotchoice
\newif\ifd@tags
\def\d@nkin@dotchoice#1{\if#1y\d@dotchoicetrue\else\d@dotchoicefalse\fi
\d@setdots}
\def\d@nkin@tags#1{\if#1y\d@tagstrue\else\d@tagsfalse\fi\d@setdots}
\def\d@setdots{%
\ifd@dotchoice
\def\d@nkinball{\e@\dynkinball\e@{\the\t@@@}}%
\ifd@tags
 \let\d@loopargs\d@loopargsa
 \let\count@rg\count@rga
 \let\init@rg\init@rga
 \let\pr@pare\pr@parea
\else
 \let\d@loopargs\d@loopargsbc
 \let\count@rg\count@rgbc
 \let\init@rg\init@rgbc
 \let\pr@pare\pr@pareb
\fi
\else
\def\d@nkinball{\dynkinball}%
\ifd@tags
 \let\d@loopargs\d@loopargsbc
 \let\count@rg\count@rgbc
 \let\init@rg\init@rgbc
 \let\pr@pare\pr@parec
\else
 \let\d@loopargs\d@loopargsd
 \let\count@rg\count@rgd
 \let\init@rg\init@rgd
 \let\pr@pare\pr@pared
\fi
\fi}

\def\d@nkin@ball#1{\e@\let\e@\dynkinball\csname d@nkin#1\endcsname}

\def\spl@ttoksa#1\@t#2\@t#3\t@end{\t@@@={#1}\t@@@@={#2}\global\t@@={#3}}%
\def\spl@ttoksb#1\@t#2\t@end{\t@@@={#1}\t@@@@={}\global\t@@={#2}}%
\def\spl@ttoksc#1\@t#2\t@end{\t@@@={}\t@@@@={#1}\global\t@@={#2}}%

\def\pr@parea{\e@\spl@ttoksa\the\t@@\t@end}%
\def\pr@pareb{\e@\spl@ttoksb\the\t@@\t@end}%
\def\pr@parec{\e@\spl@ttoksc\the\t@@\t@end}%
\def\pr@pared{\t@@{}\t@@@{}}%

\def\n@metop{\hbox to 0pt{\kern-\d@nkinrightdim\vbox to
\wd0{\vss\offinterlineskip\hsize\ht0\pr@pare
\centerline{\the\t@@@@}\kern2pt\d@nkinball}\hss}}%
%
\def\n@medown{\hbox to 0pt{\kern-\d@nkinrightdim%
\vtop to \wd0{\offinterlineskip\hsize\ht0\pr@pare%
\d@nkinball\kern2pt\centerline{\the\t@@@@}\vss}\hss}}%
%
\def\n@meright{\hbox to 0pt{\kern-\d@nkinrightdim\vtop to
\wd0{\offinterlineskip\hsize\ht0\pr@pare
\hbox{\d@nkinball\kern2pt\vbox to 
\wd0{\parindent0pt\vss\rlap{\the\t@@@@}\vss}}\vss}\hss}}%

\def\n@meleft{\hbox to 0pt{\hss\kern-\d@nkinrightdim\vtop to
\wd0{\offinterlineskip\hsize\ht0\pr@pare
\hbox{\vbox to
\wd0{\parindent0pt\vss\llap{\the\t@@@@\kern2pt}\vss}\d@nkinball}\vss}}}

\def\Tl@ne#1{\kern\d@nkinrightdim
\vbox{\hbox to #1{}\hrule}\kern\d@nkinrightdim}%
%
\def\tl@ne#1{\kern\d@nkinrightdim
\vbox{\hbox to #1{\vrule width1.5mm height.4pt
\if@ne\dimen0 1mm\else\dimen0 2mm\fi
\leaders\hbox to \dimen0{\hss.\hss}\hfill
\vrule width1.5mm height.4pt}}\kern\d@nkinrightdim
\let\hl@ne\Tl@ne}%
\def\b{\global\let\hl@ne\tl@ne}%
\def\vl@ne#1{\raise\dimen0\hbox{\vbox to #1{}\vrule}\kern-.4pt}%
%
\def\d@nkinone{\dimen9\ht0\advance\dimen9-.4pt
\raise-0.5\dimen9\n@medown}%
%
\def\d@nkinrightfork{%
\hbox{\kern\d@nkinrightdim\kern-0.1464466094\wd0
\raise-\f@rkraise
\vbox{\offinterlineskip\parindent0pt
\dimen0 0.70710678108\ht0
\if@ne
\advance\dimen0 \ht1
\else
\advance\dimen0 2\ht1
\fi
\hbox{\raise0.85355339059\wd0
\@pline%
\kern0.35355339059\wd0
\raise\dimen0
\n@meright}%
\kern-0.1464466094\ht0
\hbox{\raise0.85355339059\wd0
\d@wnline%
\kern-0.1464466094\wd0
\kern\d@nkinrightdim\n@meright}}}}%
%
\def\d@nkinleftfork{\kern.5\wd0\raise-\f@rkraise
\vbox{\offinterlineskip\parindent0pt
\dimen0 0.70710678108\ht0
\hbox{\d@wnline
\kern-2\wd1
\if@ne\dimen9 \ht1\else\dimen9 2\ht1\fi
\advance\dimen9-0.1464466094\ht0\if@ne\kern\wd1\fi
\raise\dimen9
\n@meleft}%
\kern0.70710678108\ht0
\hbox{\raise0.85355339059\wd0
\@pline%
\if@ne\kern-\wd1\else\kern-2\wd1\fi
\n@meleft}}\kern0.35355339059\wd0
\if@ne\kern\wd1  \else\kern2\wd1\fi
}%
%
\def\d@nkinright{\hl@ne\d@nkinstep\d@nkinone}%
%
\def\d@nkinup{{\vl@ne\d@nkinstep\kern0.5\wd0\raise\dimen2\n@meleft}%
\kern-0.5\wd0}%
%
\def\d@nkinuptwo{\vl@ne\d@nkinstep\kern0.5\wd0\raise\dimen2\n@meleft%
\kern-0.5\wd0\dimen9\dimen2
\advance\dimen9 0.5\ht0
\raise\dimen9\hbox{\vl@ne\d@nkinstep\kern0.5\wd0\raise\dimen2\n@meleft}%
\kern-0.5\wd0}%
%
\toksdef\t@0\toksdef\t@@1\toksdef\t@@@2%
\toksdef\t@@@@3%

\def\dynkininit#1{%
\t@{}\t@@{}\t@@@{}\t@@@@{}%
\dimendef\d@nkinstep4
\e@\d@nkinstep\d@nkinsize
%
\setbox0\hbox{\ifd@dotchoice\dynkinball{#1}\else\dynkinball\fi}%
\dimendef\d@nkinraise6
\dimendef\d@nkinrightdim7
\d@nkinrightdim\wd0
\divide\d@nkinrightdim2
%
\font\l@net=line10
\dimendef\f@rkraise3
\setbox1\hbox{\l@net\char\d@nkincount}%
\f@rkraise 1.20710678108\ht0
\advance\f@rkraise-.2pt
\if@ne
\advance\f@rkraise \ht1
\else
\advance\f@rkraise 2\ht1 
\fi
%
\dimen0\ht0
\divide\dimen0 2
\dimen2\d@nkinstep
\advance\dimen2\dimen0
%
\let\hl@ne\Tl@ne
%
\edef\@pline{\vbox{\offinterlineskip\parindent0pt\l@net
\if@ne\hsize \wd1\char\d@nkincount
\else
\hsize 2\wd1
\LINE{\hskip\wd1\char\d@nkincount\hss}\par
\char\d@nkincount\fi}}%
%
\edef\d@wnline{\vbox{\advance\d@nkincount"40\l@net
\offinterlineskip\parindent0pt\if@ne\char\d@nkincount\hsize \wd1
\else
\hsize 2\wd1
\char\d@nkincount\par
\LINE{\hskip\wd1\char\d@nkincount\hss}\fi}}%
}

\def\count@rga#1 #2,{\count255 #1\count253 #1\dynkininit{#2}\next@rg#2,}
\def\count@rgbc#1 #2 {\count255 #1\count253 #1\dynkininit{#2}\next@rg#2 }
\def\count@rgd#1 {\count255 #1\count253 #1\dynkininit{}\next@rg}
\def\init@rga#1,{\dynkininit{#1}\next@rg#1,}
\def\init@rgbc#1 {\dynkininit{#1}\next@rg#1 }
\def\init@rgd{\dynkininit{}\next@rg}

\def\d@loopargsa#1{\def\next@rg##1,##2 {\t@@=\e@{\the\t@@##1\@t##2\@t}\next}
\def\next{\ifnum\count255>1\advance\count255 -1\e@\next@rg\else#1\fi}}
\def\d@loopargsbc#1{\def\next@rg##1 {\t@@=\e@{\the\t@@##1\@t}\next}%
\def\next{\ifnum\count255>1\advance\count255 -1\e@\next@rg\else#1\fi}}
\def\d@loopargsd#1{\def\next@rg{#1}}

\def\read@rgs#1\afterread{%\t@@{}%
\d@loopargs{#1}
\ifrepe@t
\e@\count@rg
\else
\count255 \count254
\count253 \count254
\e@\init@rg
\fi}

\newif\ifrepe@t
\def\d@nkrepeat{rightrepeat}
\def\d@nkstop{st@p}
\def\d@one{1}
\def\d@right{1}
\def\d@rightrepeat{0}
\def\d@up{1}
\def\d@uptwo{2}
\def\d@rightfork{2}
\def\d@leftfork{2}

\def\countd@nkin#1,{\def\d@rep{#1}%
\ifx\d@nkrepeat\d@rep\repe@ttrue\fi\ifx\d@nkstop\d@rep\else
\advance\count254 \csname d@#1\endcsname
\e@\countd@nkin\fi}

\def\dod@nkin#1,{\def\d@rep{#1}%
\ifx\d@nkstop\d@rep\else
\csname d@nkin#1\endcsname
\e@\dod@nkin\fi}

\def\d@nkinrightrepeat{\loop
\ifnum\count253>0
\advance\count253 -1
\d@nkinright%
\repeat}

\d@setdots
\def\e@ttok#1#2\@nd{\t@@={#2}}

\def\rawdynkin#1;{\count254 0
\repe@tfalse
\countd@nkin#1,st@p,%
\bgroup
\read@rgs
\advance\count253 -\count254
%\e@\e@ttok\the\t@@\@nd
\hbox{%\kern-\d@nkinrightdim%
\dod@nkin#1,st@p,%
\kern\d@nkinrightdim}%
\egroup\afterread
}
\def\dynkinA{\rawdynkin one,rightrepeat;}
\def\dynkinD{\rawdynkin one,rightrepeat,rightfork;}
\def\dynkinDtilde#1 {\count252 #1\advance\count 252 1
\rawdynkin leftfork,one,rightrepeat,rightfork;{\count252} }
\def\dynkinE{\rawdynkin one,right,right,up,rightrepeat;}
\def\dynkinEtilde#1 {\let\d@it\relax\ifcase#1\or\or\or\or\or\or
\def\d@it{\rawdynkin one,right,right,uptwo,right,right;}\or
\def\d@it{\rawdynkin one,right,right,right,up,right,right,right;}\else
\count252 #1\advance\count 252 1
\def\d@it{\rawdynkin one,right,right,up,rightrepeat;{\count252} }\fi
\d@it}

\def\d@nkinbullet{\vbox to 3.85pt{\kern-.1pt\hbox to 3.7pt
{\kern-.43pt$\bullet$\hss}\vss}}

\def\d@nkinbulletandcirc#1{\vbox to 3.85pt{\kern-.1pt\hbox to 3.7pt
{\kern-.43pt\ifx #1c$\circ$\else$\bullet$\fi\hss}\vss}}

\def\d@nkinbigcirc{\vbox to 8.4pt{\kern-.1pt\hbox to 8.8pt
{\kern-.4pt$\bigcirc$\hss}\vss}}

\setdynkin ball=bullet
\catcode`\@=12

%%          Tests of the macros:
%%   
%%  \setdynkin size=.5cm
%%  \setdynkin lines=1
%%  \setdynkin slope="25
%%  \setdynkin tags=y
%%  
%%  \dynkinA3 1 2 3 
%%  \bigskip
%%  \setdynkin dotchoice=y
%%  \setdynkin ball=bulletandcirc
%%  \dynkinD 5 c,1 b,2 c,3 c,4 b,5 
%%  \medskip
%%  \dynkinDtilde 7 c,1 b,2 c,3 c,4 b,5 c,6 b,7 
%%  \medskip
%%  \dynkinE 10 c,1 b,2 c,3 b,4 c,5 b,6 c,7 b,8 c,9 b,10
%%  \medskip\medskip\medskip
%%  \setdynkin tags=n
%%  \dynkinEtilde 6 c b c b c b c 
%%  \medskip\medskip\medskip
%%  \setdynkin dotchoice=n
%%  \setdynkin tags=y
%%  \setdynkin ball=bullet
%%  \dynkinEtilde 7 1 2 3 4 5 6 7 8 
%%  \medskip\medskip\medskip
%%  \dynkinEtilde 8 1 2 3 4 5 6 7 8 9 
%%  \bigskip
%%  \dynkinDtilde 5 1 2 3 4 5 
%%  \medskip
%%  \setdynkin ball=bulletandcirc
%%  \setdynkin dotchoice=y
%%  \setdynkin tags=y
%%  \dynkinD7
%%  c,$\scriptstyle 1$
%%  b,$\scriptstyle 2$ 
%%  c,\b$\scriptstyle 3$
%%  b,{\hbox to 11pt{\hss$\scriptstyle n-1$}}
%%  b,{\hbox to 7pt{\hss$\scriptstyle n-2$}}
%%  b,$\scriptstyle n-1$
%%  c,$\scriptstyle n$
%%  \medskip
%%  \dynkinA3 c,1 b,2 c,3 
%%  \bigskip
%%  \dynkinDtilde7 c,1 b,2 c,3 b,4 c,5 b,6 c,7 


